Probing star clusters as cosmic ray factories

Stellar clusters (SC) are fundamental building blocks of galaxies and are among the most studied astronomical objects in the Cosmos. The recent association of diffuse $\gamma$-ray emission detected by different experiments with a dozen young SCs suggests the presence of some process able to accelerate particles at least up to hundreds of TeV. In this Ph.D. thesis, we investigate the capability of young massive stellar clusters (YMSC) to produce cosmic rays under the assumption that particles are accelerated at the cluster wind termination shock. The study is divided into three parts. First, we focus on the specific case of Cygnus OB2. We model the observed $\gamma$-ray emission (in a pure hadronic scenario) assuming different models for particle propagation in the neighborhood of the cluster. We found that particles accelerated by Cygnus OB2 can account for both the $\gamma$-ray spectrum and the radial morphology at very high energy. In the second part, we compute the diffuse $\gamma$-ray emission expected by the unresolved population of Galactic YMSC. For this purpose, we build a synthetic population of YMSC based on the properties of local SC. Under the assumption of a pure hadronic emission, we found that YMSCs can significantly contribute to the observed diffuse $\gamma$-ray emission at a few TeV. The final part of the work is dedicated to understand the impact of CRs produced by SCs on the ionization rate of molecular clouds close to those SCs. We found that the ionization rate can significantly differ from the expected value in clouds located in the unperturbed interstellar medium. We show that the measured value of ionization rate, paired with $\gamma$-ray observations, can be used to constrain particle diffusion in the vicinity of the stellar cluster.

==> CHAPTERS/acknow.tex <==
\chapter*{Acknowledgements}\label{ch:ack}
\addcontentsline{toc}{chapter}{Acknowledgements}
\markboth{Acknowledgements}{}

I would like to thank my parents who raised me since I was born, and still they are doing.




